Fixing Inventory Inaccuracies At Scale

Inaccurate records of inventory occur frequently, and by some measures cost retailers approximately 4% in annual sales. Detecting inventory inaccuracies manually is cost-prohibitive, and existing algorithmic solutions rely almost exclusively on learning from longitudinal data, which is insufficient in the dynamic environment induced by modern retail operations. Instead, we propose a solution based on cross-sectional data over stores and SKUs, observing that detecting inventory inaccuracies can be viewed as a problem of identifying anomalies in a (low-rank) Poisson matrix. State-of-the-art approaches to anomaly detection in low-rank matrices apparently fall short. Specifically, from a theoretical perspective, recovery guarantees for these approaches require that non-anomalous entries be observed with vanishingly small noise (which is not the case in our problem, and indeed in many applications). So motivated, we propose a conceptually simple entry-wise approach to anomaly detection in low-rank Poisson matrices. Our approach accommodates a general class of probabilistic anomaly models. We show that the cost incurred by our algorithm approaches that of an optimal algorithm at a min-max optimal rate. Using synthetic data and real data from a consumer goods retailer, we show that our approach provides up to a 10x cost reduction over incumbent approaches to anomaly detection. Along the way, we build on recent work that seeks entry-wise error guarantees for matrix completion, establishing such guarantees for sub-exponential matrices, a result of independent interest.

==> sections/acknowledge.tex <==
\section{Acknowledgement}

We thank all anonymous reviewers for their constructive comments. Farias and Peng were partially supported by NSF Grant CMMI 1727239.

==> sections/minimax.tex <==
\section{Minimax Lower Bound} \label{sec:lower}
In this section, we provide a sketch for showing \cref{prop:lower-bound} based on the hypothesis testing argument.  Recall that an model is specified by $p_{\O}, p_{\A}^{*}, \alpha^{*}, M^{*}$, and the anomaly distribution $\Ano(\cdot, \cdot).$ We consider the following special model:
\begin{itemize}
\item All the entries can be observed, i.e., $p_{\O}=1.$
\item When the anomaly occurs, $X_{ij} = 0,$ i.e., $\Probx{\Ano}{X_{ij}=0~|~M} = 1$ for any $M \in \R_{\geq 0}.$  
\end{itemize} 
This corresponds to the scenario that ``extreme phantom inventory'' occurred, e.g., items being broken or stealing without notice. We also choose $p_{\A}^{*}=1/2$ ($\alpha^{*}$ is not needed in this model). We will show that even for this simple anomaly model, one cannot expect regret on TPR better than $O(1/\sqrt{n}).$

The difficulties of achieving the optimal $\TPR$ are rooted on the difficulties of recovering the exact $M^{*}$ based on $X$. Hence, we construct a set of matrices that are particular difficult to identify given the observation $X$. Specifically, for any even number $n$, we construct $\mathcal{M}_n =\{M^{b} \in \R^{n\times n}, b \in \{0,1\}^{n/2} \}$ as follows. Fix a constant $C$. Consider $n \geq 4C^2$ and $b \in \{0, 1\}^{n/2}$. For any $i \in [n/2], j \in [n]$,  
\begin{itemize}
\item if $b_{i} = 0$, $M^{b}_{2i,j} = 1$ and $M^{b}_{2i+1,j} = 1 - \frac{C}{\sqrt{n}};$
\item if $b_{i} = 1$, $M^{b}_{2i,j} = 1 - \frac{C}{\sqrt{n}}$ and $M^{b}_{2i+1,j} = 1.$
\end{itemize}
Therefore, $M^{b}$ consists of two possible values: $1$ or $1-\frac{C}{\sqrt{n}}.$ The entries of the same row of $M^{b}$ have the same values. The $b_i$ indicates the allocation of $1$ and $1-\frac{C}{\sqrt{n}}$ over the $2i$-th row and the $(2i+1)$-th row of $M^{b}.$ 

Let $\Pi_\gamma$ denote the set of all policies $\pi$ such that 
$\Probx{X|M^{b}}{\FPR_{\pi}(X) \leq \gamma} \geq 1-C/n^2$ for all $M^{b} \in \mathcal{M}_{n}.$ We will establish \cref{prop:lower-bound} by showing that, with $\gamma = \frac{1}{2e}$, for any algorithm $\pi \in \Pi_\gamma$, there exists $M' \in \mathcal{M}_{n}$ such that $\Ex{X|M'}{\TPR_{\pi^{*}(\gamma)}(X) - \TPR_{\pi}(X)} \geq  C/\sqrt{n}$. 

Note that for a rational policy $\pi$, due to the ``extreme phantom inventory'' model, the anomaly will be claimed (i.e., $A^{\pi}_{ij}=1$) only when $X_{ij} = 0$ is observed. We then have the following lemma, stating that the overall probability for claiming anomaly is bounded due to FPR constraints. 
\begin{lemma} For any $\pi \in $

\end{lemma}


Consider $M^{b_1}$ and $M^{b_2}$ where $b_1$ and $b_2$ only differ in one bit. Let $X^{b_1}$ and $X^{b_2}$ be the observation generated from $M^{b_1}$ and $M^{b_2}$ respectively. Due to our construction, one can verify that the KL-divergence between $X^{b_1}, X^{b_2}$ is small, i.e. $D_{KL}(X^{b_1} || X^{b_2}) \approx 0.$

the probability of successfully distinguishing $b_1$ and $b_2$ is small. 

Let $x^{+} = 1, x^{-} = 1 - \frac{c}{\sqrt{n}}.$ For any $M \in \mathcal{M}_{n}$, by the construction, there are one-half entries of $M$ with values $x^{+}$ and one-half entries with values $x^{-}$. Note that, when observing $X_{ij} = 0$, $\pi^{*}$ would claim anomaly on the entry $x^{+}$ with priority than $x^{-}$, because it is more possible to observe $0$ for $x^{-}$ in the normal situation. Indeed, we choose $\gamma$ and $p_{\A}^{*}$ in a way that $\pi^{*}$ roughly claims anomalies for all $x^{+}$ entries with $X_{ij}=0$.

Intuitively speaking, if an algorithm $\pi$ achieves the similar performance as $\pi^{*}$, it must be able to distinguish $M^{+}$ and $M^{-}$ from the observation $X$. However, the construction of $\mathcal{M}_{n}$ prevent this distinguishability. Consider $M^{b_1}$ and $M^{b_2}$ where $b_1$ and $b_2$ only differs in one element. Then one can verify that $\Probx{X\sim \mathrm{H}(p_{\A}^{*}, M^{b_1})}{X \in A} \approx \Probx{X\sim \mathrm{H}(p_{\A}^{*}, M^{b_2})}{X\in A}$ for any set $A$. This finally leads to the $O(\frac{1}{\sqrt{n}})$ regret between $\pi$ and $\pi^{*}.$ 


For any $M^{b} \in \mathcal{M}_{n},$ one can verify that the assumptions in \cref{sec:model} hold for $X \sim \mathrm{H}(p_{\A}^{*}, M^{b})$. In particular,
\begin{itemize}
\item $L = O(1)$ because $\norm{M^{b}}_{\max} \leq 1$ and $\norm{\Ano(M)}_{\psi_1} = 0$ for $M \in \R_{\geq 0}.$  
\item $K=O(1)$ because $\Prob{\Ano(M)=k}$ is independent of $M$ for $k \in \mathbb{N}$ and $M \in \R_{\geq 0}.$
\item $\kappa, \mu, r = O(1).$ Note that $M^{b}$ has the decomposition $M_{ij}^{b} = x_{i} y_{j}$ where $x, y \in \R^{n}.$ In particular, one can verify that for $j \in [n]$, $y_{j} = 1$; and for $i \in [n/2]$, $x_{2i} = 1 - (\frac{C}{\sqrt{n}})^{b_i}, x_{2i+1} = 1-(\frac{C}{\sqrt{n}})^{1-b_i}$.
Hence, $M^{b}$ is rank-1 ($r=1$) and has $\kappa = \sigma_1^{*}/\sigma_{r}^{*} =1.$ To consider $\mu$, note that the SVD decomposition of $M^{b}$ is $M^{b}=\frac{x}{\norm{x}} (\norm{x}\norm{y}) \frac{y^{T}}{\norm{y}}$ where $\frac{x}{\norm{x}}$ and $\frac{y}{\norm{y}}$ are two singular vectors. Observing that $\frac{x_i}{\norm{x}} \leq \frac{1}{\sqrt{n}(1-\frac{C}{\sqrt{n}})} \leq \frac{2}{\sqrt{n}}, \frac{y_j}{\norm{y}} \leq \frac{1}{\sqrt{n}}.$
Therefore, $\mu = O(1)$ for $M^{b}.$
\end{itemize}
The regularity conditions (RC) also can be verified easily. By \cref{thm:main-theorem}, an TPR regret with $O(n^{-1/2}\log^{1.5}(n))$ can be achieved. 



We consider the following special model: let $p_{\O}=1$ and $p_{\A}^{*} = \frac{1}{2}$, and when $B_{ij}=1$, $X_{ij}=0.$ We refer to this in notational form as $X\sim \mathrm{H}(M^{*})$.

We construct $\mathcal{M}_n =\{M^{b} \in \R^{n\times n}, b \in \{0,1\}^{n/2} \}$ as follows. Fix a constant $C$. Consider $b \in \{0, 1\}^{n/2}$. For any $i \in [n/2], j \in [n]$,  if $b_{i} = 0$, $M^{b}_{2i,j} = 1$ and $M^{b}_{2i+1,j} = 1 - \frac{C}{\sqrt{n}};$ if $b_{i} = 1$, $M^{b}_{2i,j} = 1 - \frac{C}{\sqrt{n}}$ and $M^{b}_{2i+1,j} = 1.$ Let $M^{b}$ be drawn uniformly form $\mathcal{M}_{n}$ and $X \sim \mathrm{H}(M^{b}).$ In order to achieve high $\TPR$, one needs to identify the correct $b$ given $X$. By our construction, the error probability for distinguishing $M^{b_1}$ and $M^{b_2}$ is large when $b_1$ is 1-bit different from $b_2$. This provides a lower bound on identifying $b$ and leads to a $O(1/\sqrt{n})$ regret on $\TPR$. The formal proof can be found in the Appendix. One can also verify that \cref{thm:main-theorem} guarantees $O(\log^{1.5} n / \sqrt{n})$ regret for every $M^{b} \in \mathcal{M}_{n}.$ This shows that our algorithm is optimal for the TPR up to logarithmic factors. 

%
%For any $M^{b} \in \mathcal{M}_{n},$ one can verify that the assumptions in \cref{sec:model} hold for $X \sim \mathrm{H}(p_{\A}^{*}, M^{b})$. In particular,
%\begin{itemize}
%\item $L = O(1)$ because $\norm{M^{b}}_{\max} \leq 1$ and $\norm{\Ano(M)}_{\psi_1} = 0$ for $M \in \R_{\geq 0}.$  
%\item $K=O(1)$ because $\Prob{\Ano(M)=k}$ is independent of $M$ for $k \in \mathbb{N}$ and $M \in \R_{\geq 0}.$
%\item $\kappa, \mu, r = O(1).$ Note that $M^{b}$ has the decomposition $M_{ij}^{b} = x_{i} y_{j}$ where $x, y \in \R^{n}.$ In particular, one can verify that for $j \in [n]$, $y_{j} = 1$; and for $i \in [n/2]$, $x_{2i} = 1 - (\frac{C}{\sqrt{n}})^{b_i}, x_{2i+1} = 1-(\frac{C}{\sqrt{n}})^{1-b_i}$.
%Hence, $M^{b}$ is rank-1 ($r=1$) and has $\kappa = \sigma_1^{*}/\sigma_{r}^{*} =1.$ To consider $\mu$, note that the SVD decomposition of $M^{b}$ is $M^{b}=\frac{x}{\norm{x}} (\norm{x}\norm{y}) \frac{y^{T}}{\norm{y}}$ where $\frac{x}{\norm{x}}$ and $\frac{y}{\norm{y}}$ are two singular vectors. Observing that $\frac{x_i}{\norm{x}} \leq \frac{1}{\sqrt{n}(1-\frac{C}{\sqrt{n}})} \leq \frac{2}{\sqrt{n}}, \frac{y_j}{\norm{y}} \leq \frac{1}{\sqrt{n}}.$
%Therefore, $\mu = O(1)$ for $M^{b}.$
%%\end{itemize}
%Choose $T=1$, the regularity conditions (RC) also can be verified (see details in the Appendix \ref{sec:lower-bound-appendix}). By the \cref{thm:main-theorem}, we can obtain
%\begin{proposition}\label{prop:upper-bound}
%For any $M^{b} \in \mathcal{M}_{n}$, let $X \sim \mathrm{H}(p_{\A}^{*}, M^{b})$. With probability $1-O(1/n^2),$ 
%\begin{align*}
%\FPR_{\pi^{\AD}(\gamma)}(X) &\leq \gamma, \\
%\TPR_{\pi^{\AD}(\gamma)}(X) &\geq \TPR_{\pi^{*}(\gamma)}(X) - C\frac{\log^{1.5}(n)}{\sqrt{n}}.
%\end{align*}  
%\end{proposition}
%
%Next, we provide a proof sketch for \cref{prop:lower-bound} based on the construct of $\mathcal{M}_{n}$. The full details can be found in Appendix \ref{sec:lower-bound-appendix}.
%\begin{proof}[Proof Sketch of \cref{prop:lower-bound}]
%Let $C_1, C_2$ be two constants. 
%To allow for comparison to \cref{prop:upper-bound}, let $\Pi_\gamma$ denote the set of all policies $\pi$ such that 
%%On the other hand, our algorithm achieves $O(\log n/\sqrt{n})$ regret for a broad class of anomaly models, which demonstrates its applicability.
%$    \Probx{X\sim \mathrm{H}(p_{\A}^{*}, M^{b})}{\FPR_{\pi}(X) \leq \gamma} \geq 1-C_1/n^2
%$
%for all $M^{b} \in \mathcal{M}_{n}.$
%
%We aim to show that for any algorithm $\pi \in \Pi_\gamma$, there exists $M' \in \mathcal{M}_{n}$ such that
%\begin{align*}
%    \Ex{X\sim \mathrm{H}(p_{\A}^{*}, M')}{\TPR_{\pi^{*}(\gamma)}(X) - \TPR_{\pi}(X)} \geq  \frac{C_2}{\sqrt{n}}.
%\end{align*}
%This concrete statement is sufficient to show the \cref{prop:lower-bound}.
%
%Let $M^{+} = 1, M^{-} = 1 - \frac{C}{\sqrt{n}}.$ For any $M \in \mathcal{M}_{n}$, there are one-half $M^{+}$ and one-half $M^{-}$ entries in $M$. Note that, when observing $X_{ij} = 0$, $\pi^{*}$ would claim anomaly on the entry $M^{+}$ with priority than $M^{-}$, because it is more possible to observe $0$ for $M^{-}$ in the normal situation. Indeed, we choose $\gamma$ and $p_{\A}^{*}$ in a way that $\pi^{*}$ roughly claims anomalies for all $M^{+}$ entries with $X_{ij}=0$.
%
%Intuitively speaking, if an algorithm $\pi$ achieves the similar performance as $\pi^{*}$, it must be able to distinguish $M^{+}$ and $M^{-}$ from the observation $X$. However, the construction of $\mathcal{M}_{n}$ prevent this distinguishability. Consider $M^{b_1}$ and $M^{b_2}$ where $b_1$ and $b_2$ only differs in one element. Then one can verify that $\Probx{X\sim \mathrm{H}(p_{\A}^{*}, M^{b_1})}{X \in A} \approx \Probx{X\sim \mathrm{H}(p_{\A}^{*}, M^{b_2})}{X\in A}$ for any set $A$. This finally leads to the $O(\frac{1}{\sqrt{n}})$ regret between $\pi$ and $\pi^{*}.$ 
%\end{proof}




==> sections/preliminaries.tex <==

\section{Model and Problem Statement}

We begin by introducing our model for the phantom inventory problem that will be studied throughout this paper. While we will focus on this single application for the sake of concreteness, our model is substantially more general, as we will note throughout. 

\subsection{An Observational Model for Phantom Inventory}

\input{sections/preliminaries_model.tex}

For a brief moment, consider a {\em single} product $j$ being sold at a {\em single} store $i$. The sales of this product is typically modeled as a Poisson process, and thus during a fixed time period of interest (the previous week, say), the number of units sold can reasonably be represented as a Poisson variable with (unknown) mean $M_{ij}^*$. However, this assumes proper {\em merchandising}, meaning that the product is available and in the physical in-store location we expect. In reality, errors in merchandising happen often and for a variety of reasons (misplacement, theft, etc.), resulting in lower sales due to inventory being missing when expected to exist. These occurrences of {\em phantom inventory} are precisely the anomalies we seek to detect, and while it would seem impossible to detect such an anomaly through any means other than brute-force (sending an employee to manually verfiy), we will leverage the fact that this problem usually occurs simultaneously across {\em multiple} products and stores.

Consider now a retailer selling $m$ different products across $n$ stores. The retailer observes a sales matrix $X \in \R^{n \times m}$, where $X_{ij}$ is the number of units of product $j$ sold at store $i$. We assume that $X$ is generated according to a model with three sets of values that are initially unknown: 
\begin{enumerate}
	\item (Non-anomaly sales) An $r$-rank matrix $M^{*} \in \R^{n \times m}$ (assume $n\leq m$ without loss of generality), where $M^{*}_{ij}$ equals the expected sales for the $j$-th product at the $i$-th store, assuming no merchandising error. 
	\item (Anomaly occurrences)  A binary matrix $B \in \R^{n\times m}$ such that $B_{ij} = 1$ if and only if an anomaly has occurred at entry $(i,j)$. This matrix $B$ is the main object we are interested in estimating. We assume that its entries are drawn independently from a Bernoulli distribution with unknown mean $p_a^{*}$. 
	\item (Anomaly model) A vector $\alpha^{*} \in \R^{d}$ which parameterizes the sales distribution under an anomaly. The distribution of sales at entry $(i,j)$ under an anomaly is given by a non-negative, integer-valued distribution $\mathrm{Anom}(\alpha^{*}, M_{ij}^{*})$. 
\end{enumerate}
Finally, to allow for the sales of certain product-store pairs to be unobserved or `missing' (e.g. because the product is not offered at the store), we let $\Omega \subset [n]\times[m]$ denote the subset of entries of $X$ that are actually observed. In our theoretical analysis, we will assume that each entry is observed independently with probability $p_{o}$. 

To summarize, the sales matrix $X$ is generated according to
\begin{align} X_{ij} \sim
 \begin{cases}  \Pos(M_{ij}^{*}) & \text{if } B_{ij} = 0 \\ 
 \Ano(\alpha^{*}, M_{ij}^{*}) & \text{if } B_{ij} = 1.
\end{cases}
\end{align}
%where $Poisson(M_{ij}^{*})$ is the Poisson distribution with the mean $M^{*}_{ij}$ and . 
%Let $\Omega = \{(i, j)~|~O_{ij}=1\}$ where $O_{ij} \sim \Ber(p_{o})$. The observation is $(X, \Omega)$, where $X_{ij}= X'_{ij}$ if $(i,j) \in \Omega$ otherwise $0$. 
Given $X_\Omega$, our goal is to infer $B$ (i.e., the position of anomalies). We refer to this model as the phantom inventory model, written as $X_\Omega \sim \mathrm{PI}(M^{*}, \alpha^{*}, p_a^{*}, p_o)$.

Before moving on to describe the anomaly detection problem, it is worth stating the assumptions we will make on the phantom inventory model. First, with respect to $M^*$: let $M^{*} = U \Sigma V^{T}$, be the SVD, where $\Sigma \in \R^{r\times r}$ is a diagonal matrix with singular values $\sigma_1^{*} \geq \sigma_2^{*} \geq \dotsc \geq \sigma_{r}^{*}$; and $U \in \R^{n \times r}, V \in \R^{m \times r}$ are two matrices that hold the left and right-singular vectors.  We make the following assumptions:
\begin{itemize}
    \item(Boundedness): $\norm{M^{*}}_{\max} \leq L.$ 
    \item (Incoherence): $\norm{U}_{2,\infty}^2 \leq \frac{\mu r}{n}, \norm{V}_{2,\infty}^2 \leq \frac{\mu r}{m}$. \footnote{For $A \in \R^{n\times m}$, $\norm{A}_{2,\infty} := \max_{i \in [n]}\sqrt{\sum_{j\in[m]} A_{ij}^2}$.}%, where $\mu$ and $r$ is small compared to $n.$
    \item (Minimum total sales): $\sum_{i,j} M_{ij}^{*} \geq C\frac{n^2}{p_o \log m}.$
\end{itemize}
Similar to existing results in matrix completion and recovery, our guarantees will be parameterized by $\mu$, $L$, and $\kappa = \sigma_1^{*}/\sigma_{r}^{*}.$
%One of typical scenarios we considered is $\kappa=O(1),r=O(1),\mu=O(1),L=O(1)$. See details below for more general conditions. 

Our other set of assumptions is for the sales distribution under anomaly:
\begin{itemize}
    %\item{Assumption} (independence): noise, anomalies, observations occur i.i.d. 
    %\item{Assumption} (boundedness on anomalies): $p_a$ is a constant.
    \item(Sub-exponential) $\Ano(\alpha^{*},m)$ is sub-exponential: $\norm{\Ano(\alpha^{*},m)}_{\psi_1} \leq L.$\footnote{The sub-exponential norm of $X$ is defined as 
   $ \norm{X}_{\phi_1} := \inf\{t > 0: \E{\exp(|X|/t)}\leq 2\}.$
}  

    \item(Linear scaling) There exists function $g$ such that $\E{\mathrm{Anom}(\alpha^{*},m)} = g(\alpha^{*})m$.%Suppose $T \sim Anomaly(\vec{\alpha}, \tilde{m})$. Then $T$ is subexponential random variable with $E[T] = g(\vec{\alpha}) \tilde{m}$ and         \item $g(\vec{\alpha}, M;X) = P_{Anomaly}(X|\vec{\alpha}, M)$ is $K$-Lipschitz (given any $X$):
    \item(Lipschitz) For any $\alpha_1$,$\alpha_2$,$M_1$,$M_2$,
    \begin{align}
        |\Probx{\Ano}{X|\vec{\alpha}_1, M_1} - \Probx{\Ano}{X|\vec{\alpha}_2, M_2}| \leq K\norm{(\alpha_1-\alpha_2, M_1 - M_2)}_2 
    \end{align}
  \end{itemize}

One natural choice is to take $\alpha$ to be a single parameter in $[0,1)$, and let the distribution be Poisson with mean $\alpha^{*} M^*_{ij}$.
%\begin{definition}[Sub-exponential norm]
%The sub-exponential norm of $X$, denoted by $\norm{X}_{\phi_1}$, is 
%\begin{align}
%    \norm{X}_{\phi_1} := \inf\{t > 0: \E{\exp(|X|/t)}\leq 2\}.
%\end{align}
%\end{definition}




\subsection{Performance Measure: The Receiver Operating Characteristic (ROC) Curve}
Given an observation $X$, an algorithm $\pi$ outputs $A_{ij}^{\pi}(X)$ to specify whether an anomaly occurs in the position $(i, j).$ One can view the goal of $\pi$ as aiming to correctly classify the entries into ``anomaly set'' and ``non-anomaly set''. 

In a classification task, the metric ``true positive rate'' and ``false positive rate'' are commonly used to characterize the performance of algorithms. In particular, we call an entry $(i, j)$ ``positive'' if $B_{ij} = 1$; ``negative'' if $B_{ij} = 0.$ Furthermore, an entry $(i, j)$ is called ``true positive'' if $A_{ij}^{\pi}(X) = 1$ and $B_{ij} = 1$; ``false positive'' if $A_{ij}^{\pi}(X) = 1$ and $B_{ij} = 0.$

Let $\Omega = \{(i, j)\}$ be the observing entries in $X$, we have the following definition. 
\begin{definition}
The true positive rate (TPR) of an algorithm $\pi$ given an observation $X$ is denoted by
\begin{align}
    \TPR_{\pi}(X) := \frac{\E{\sum_{(i, j)\in \Omega}\1{A_{ij}^{\pi}(X)=1, B_{ij} = 1}}}{\E{\sum_{(i,j)\in \Omega} \1{B_{ij}=1}}},
\end{align}
i.e., the ratio between the expected number of true positive samples $TP^{\pi}(X)$ over the expected number of positive samples $N^{pos}(X)$. Similarly, the false positive rate (FPR) of a policy $\pi$ given an observation $X$ is denoted by
\begin{align}
    \FPR_{\pi}(X) := \frac{\E{\sum_{(i,j)\in \Omega}\1{A_{ij}^{\pi}(X)=1, B_{ij} = 0}}}{\E{\sum_{(i,j) \in \Omega} \1{B_{ij}=0}}}, 
\end{align}
i.e., the ratio between the expected number of false positive samples $FP^{\pi}(X)$ over the expected number of negative samples $N^{neg}(X)$.\footnote{We suppose $TPR_{\pi}(X) = 0$ if $E\{\sum_{(i,j)\in \Omega} 1\{B_{ij}=1\}\} = 0$; $FPR_{\pi}(X) = 0$ if $E\{\sum_{(i,j)\in \Omega} 1\{B_{ij}=0\}\} = 0$.} 

\end{definition}

Let $f^{*}_{ij}$ be the probability that an entry does not have an anomaly given the observation $X$. In particular $f_{ij}^{*} := \Prob{B_{ij} = 0~|~X} = \frac{y_{ij}}{x_{ij}+y_{ij}}$, where 
$x_{ij} := p_a^{*} \Probx{\Ano}{X_{ij}|\vec{\alpha}^{*}, M_{ij}^{*}}, y_{ij} := (1-p_a^{*}) \Probx{\Pos}{X_{ij}|M_{ij}^{*}}.$ We have the following result by some algebra. 
\begin{align}
    \TPR_{\pi}(X) &= \frac{\sum_{(i, j) \in \Omega}\Prob{A_{ij}^{\pi}(X)=1}(1-f_{ij}^{*})}{\sum_{(i,j) \in \Omega} (1-f_{ij}^{*})} \label{eq:TPR-equation}\\
    \FPR_{\pi}(X) &= \frac{\sum_{(i, j) \in \Omega} \Prob{A_{ij}^{\pi}(X)=1} f_{ij}^{*}}{\sum_{(i,j) \in \Omega} f_{ij}^{*}}. \label{eq:FPR-equation} 
\end{align}
Intuitively, we want to maximize the TPR while maintaining a low FPR.

\subsection{Prior Approaches}
